AERO: Audio Super Resolution in the Spectral Domain

We present AERO, a audio super-resolution model that processes speech and music signals in the spectral domain. AERO is based on an encoder-decoder architecture with U-Net like skip connections. We optimize the model using both time and frequency domain loss functions. Specifically, we consider a set of reconstruction losses together with perceptual ones in the form of adversarial and feature discriminator loss functions. To better handle phase information the proposed method operates over the complex-valued spectrogram using two separate channels. Unlike prior work which mainly considers low and high frequency concatenation for audio super-resolution, the proposed method directly predicts the full frequency range. We demonstrate high performance across a wide range of sample rates considering both speech and music. AERO outperforms the evaluated baselines considering Log-Spectral Distance, ViSQOL, and the subjective MUSHRA test. Audio samples and code are available at https://pages.cs.huji.ac.il/adiyoss-lab/aero

==> hop_length_table.tex <==
% \begin{table*}[tp!]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{\hskip6pt}c|ccc|ccc|ccc|ccc} 
%     \toprule
%      & 
%      \multicolumn{3}{|c|}{8-16} & 
%      \multicolumn{3}{|c|}{8-24} & 
%      \multicolumn{3}{|c|}{4-16} & 
%      \multicolumn{3}{|c}{11-44} \\
%     \midrule
%      & $\downarrow$ & $\uparrow$ & $\uparrow$ \
%      & $\downarrow$ & $\uparrow$ & $\uparrow$ \
%      & $\downarrow$ & $\uparrow$ & $\uparrow$ \
%      & $\downarrow$ & $\uparrow$ & $\uparrow$ \\     
%     \midrule
%         Ours ($\nicefrac{256}{512}$) & - & - & - & 0.992 & 4.033 & 98.76 & 1.04 & 3.036 & 84.72 & - & - & - \\
%         Ours ($\nicefrac{128}{512}$) & - & - & - & 0.913 & 4.122 & 96 & 0.987 & 3.152 & 95.08 & - & - & - \\
%         Ours ($\nicefrac{64}{512}$)  & 0.772 & 4.158 & 95.246 & 0.9 & 4.167 & 94.36 & 0.943 & 3.275 & 92.48 & 1.107 & - & - \\
%     \bottomrule
% \end{tabular}
% \label{tab:hop_length_results}
% }
% \vspace{0.5em}
% \caption{Comparison of hop-length parameters}
% \end{table*}


==> related_work.tex <==
\section{Related Work}
\label{sec:related}
\ortal{to my opinion this could be either discarded if intoduction includs enough elabration or moved to the end of the paper}
% Demucs, Hybrid Demucs
Demucs \cite{defossez2020real} \cite{hdemucs} is a convolutional U-net architecture, with an attention module placed between the encoder and decoder. It has demonstrated great performance on source separation and audio denoising.

% Super-Resolution works:

% Nu-GAN, this is an important comparison - as it is also a GAN that operates in the spectral domain.
% With respect to Nu-GAN, we use both imaginary and real components of STFT - therefore using also the phase. We upsample in the spectral domain.

% Previous work has put much effort in delibirately estimating the phase information \cite{phase-aware} or flipping the input phase \cite{li, eskimez}, we avoid this by using the Complex-as-channels approach.

% Previous work \cite{li, eskimez} concatenate the low-frequency input features with the generated high-frequency output, our spectral upsampling technique avoids the need for this.

\cite{nugan} applies an adversarial method in the frequency domain, by predicting the residual spectrogram of the missing high frequencies from 22Khz to 44Khz.

% T-Film, Audio-Super-Resolution: Basic U-Net Architecture

\cite{kuleshov} has shown good results on \ac{SSR} using a simple convolutional u-net architecture. \cite{tfilm} has improves upon this work, using a temporal FiLM module.

% SeaNET: Adversarial method that works well in the waveform domain

\cite{seanet} has shown great performance on \ac{SSR} by applying an adversarial method in the waveform domain.

% Nu-Wave/Nu-wave2: diffusion models. Nuwave2 works on different sampling rates.
\cite{nuwave} has adapted audio diffusion methods to upsample from 16 and 24 Khz to 48 Khz. \cite{nuwave2} has improved upon this work, and showed results on \ac{SSR} from different low sampling rates to 48 Khz.

% VoiceFixer: General speech enhancement system. Works on different augmentations, and upsampling rates.
\cite{voicefixer} combines a variety of modules into a generative framework that tackles the general speech restoration task: simultaneously improving denoising, dereverbaration, declipping, and super-resolution in a single task. \moshe{this citation might be redundant.}



==> results_table.tex <==

% \begin{table}[h!]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{\hskip6pt}c|c|ccc} 
%     \toprule
%      & Method & LSD $\downarrow$ & VISQOL $\uparrow$ & MUSHRA $\uparrow$ \\
%     \midrule
%         \multirow{5}{*}{\rotatebox[origin=c]{90}{8-16 KHz}}
%         & Reference & - & - & 95.230 \\
%         & Anchor & - & - & 66.068 \\
%         \cmidrule{2-5}
%         & Sinc & 2.322 & 3.412 & 71.418 \\
%         & TFiLM~\cite{kuleshov} & 1.271 & 3.181 & 69.777 \\
%         & SEANet~\cite{seanet} & 0.794 & 4.078 & 94.726 \\
%         \cmidrule{2-5}
%         & Ours ($\nicefrac{256}{512}$) & - & - & - \\
%         & Ours ($\nicefrac{128}{512}$) & - & - & - \\
%         & Ours ($\nicefrac{64}{512}$) & \bf{0.772} &\bf{4.158} & \bf{95.923} \\
%     \midrule
%         \multirow{4}{*}{\rotatebox[origin=c]{90}{8-24 KHz}}
%         & Reference & - & - & 98.25 \\
%         & Anchor & - & - & 45.45 \\
%         \cmidrule{2-5}
%         & Sinc & 2.959 & 3.414 & 53.2 \\
%         & SEANet~\cite{seanet} & 0.911 & 4.059 & 94.8 \\
%         \cmidrule{2-5}
%         & Ours ($\nicefrac{256}{512}$) & - & - & 99.4 \\
%         & Ours ($\nicefrac{128}{512}$) & 0.913 & 4.122 & 96.8 \\
%         & Ours ($\nicefrac{64}{512}$) & - & - & 95.5 \\
%     \midrule
%         \multirow{5}{*}{\rotatebox[origin=c]{90}{4-16 KHz}}
%         & Reference & - & - & 96.68 \\
%         & Anchor & - & - & 32.8 \\
%         \cmidrule{2-5}
%         & Sinc & 3.586 & 2.27 & 33.24 \\
%         & TFiLM~\cite{kuleshov} & 1.774 & 2.253 & 33.44 \\
%         & SEANet~\cite{seanet} & 0.986 & 3.158 & 91.08 \\
%         \cmidrule{2-5}
%         & Ours ($\nicefrac{256}{512}$) & 1.04 & 3.036 & 84.72 \\
%         & Ours ($\nicefrac{128}{512}$) & 0.987 & 3.152 & 95.08 \\
%         & Ours ($\nicefrac{64}{512}$) & \bf 0.943 & \bf 3.275 & 92.48 \\
%     \midrule
%         \multirow{5}{*}{\rotatebox[origin=c]{90}{12-48 KHz}}
%         & Reference & - & - & 100 \\
%         & Anchor & - & - & 63.5 \\
%         \cmidrule{2-5}
%         & Sinc & 3.355 & 4.328 & 66.95 \\
%         & SEANet~\cite{seanet} & 0.861 & 4.712 & 99 \\
%         & NuWave2~\cite{nuwave2} & 1.336 & 4.423 & 82.4 \\
%         \cmidrule{2-5}
%         & Ours ($\nicefrac{256}{1024}$) & 0.915 & 4.667 & 99.25 \\
%     \midrule
%         % \multirow{5}{*}{\begin{tabular}{@{}c@{}}(MusDB) \\ 11-44 KHz\end{tabular}}
%         \multirow{5}{*}{\rotatebox[origin=c]{90}{(MusDB) 11-44 KHz}}
%         & Reference & - & - & - \\
%         & Anchor & - & - & - \\
%         \cmidrule{2-5}
%         & Sinc & 3.913 & 1.97 & - \\
%         & SEANet~\cite{seanet} & 1.131 & 2.88 & - \\
%         & BehmGAN~\cite{behmgan} & 1.797 & 2.01 & - \\
%         \cmidrule{2-5}
%         & Ours ($\nicefrac{256}{512}$) & - & - & - \\
%         & Ours ($\nicefrac{128}{512}$) & 1.157 & 2.893 & - \\
%         & Ours ($\nicefrac{64}{512}$) & - & - & - \\
%     \bottomrule
%     \end{tabular}}
% \label{tab:results}
% \vspace{0.5em}
% \caption{Results}
% \end{table}
